The NANOGrav Nine-year Data Set: Observations, Arrival Time Measurements, and Analysis of 37 Millisecond Pulsars

We present high-precision timing observations spanning up to nine years for 37 millisecond pulsars monitored with the Green Bank and Arecibo radio telescopes as part of the North American Nanohertz Observatory for Gravitational Waves (NANOGrav) project. We describe the observational and instrumental setups used to collect the data, and methodology applied for calculating pulse times of arrival; these include novel methods for measuring instrumental offsets and characterizing low signal-to-noise ratio timing results. The time of arrival data are fit to a physical timing model for each source, including terms that characterize time-variable dispersion measure and frequency-dependent pulse shape evolution. In conjunction with the timing model fit, we have performed a Bayesian analysis of a parameterized timing noise model for each source, and detect evidence for excess low-frequency, or "red," timing noise in 10 of the pulsars. For 5 of these cases this is likely due to interstellar medium propagation effects rather than intrisic spin variations. Subsequent papers in this series will present further analysis of this data set aimed at detecting or limiting the presence of nanohertz-frequency gravitational wave signals.

==> contrib.tex <==
An alphabetical-order author list was used for this paper in recognition
of the fact that a large, decade-timescale project such as this is
necessarily the result of the work of many people.  All co-authors of
this paper actively contribute to the scientific activities of the
NANOGrav collaboration and as such are all directly responsible for
these results.  All co-authors reviewed the manuscript text and figures
prior to the paper's submission.  Certain specific contributions to this
paper include:
ZA, KC, PBD, TD, RDF, EF, MEG, GJ, MJ, MTL, LL, MAM, DJN, TTP, SMR, IHS,
KS, JKS, and WWZ all ran observations during which these data were
collected, and fit timing models to the TOA data as described in
\S\ref{sec:timing}.
EF authored the manuscript text for \S\ref{sec:intro} and
\S\ref{sec:timing}.  
DJN authored \S\ref{sec:obs} and created
Table~\ref{tab:obs:observing_systems} and Figure~\ref{fig:obs:epochs}.  
PBD authored \S\ref{sec:toa} and perfomed the calibration and TOA
generation; authored \S\ref{sec:conclusions}; authored
Appendices~\ref{sec:offset} and \ref{sec:snr} and performed the analyses
described there; created Tables~\ref{tab:psr_params},
\ref{tab:timingpar}, and \ref{tab:offsets}; created
Figures~\ref{fig:fd}, \ref{fig:offsets}, \ref{fig:toa_pdf} and
\ref{fig:resid_snr}; and compiled the data files for public release.
JAE authored \S\ref{sec:noise} and Appendix~\ref{sec:noise_app} and
performed the noise analysis; authored Appendix~\ref{sec:daily_avg}; and
created Figure~\ref{fig:red-comp} and
Figures~\ref{fig:summary-J0023+0923} through
\ref{fig:summary-J2317+1439}.
ZA, JMC, TD, IHS, SMR and (others?) edited the manuscript text and/or
provided significant input about its content.


==> table_epochs.tex <==
\begin{table*}
\label{tab:epochs}
\caption{Number of Epochs of Observation by Pulasr and Observing System (xxx need to sort columns by frequency and replace labels like L-wide with frequency labels}
\begin{tabular}{lcccccccccccc}
\hline
\hline
& 327 & 327 & 430 & 430 & L-wide & L-wide & Rcvr1-2 & Rcvr1-2 & Rcvr-800 & Rcvr-800 & S-wide & S-wide \\
\multicolumn{1}{c}{Pulsar}  & ASP & PUPPI & ASP & PUPPI & ASP & PUPPI & GASP & GUPPI & GASP & GUPPI & ASP & PUPPI \\
& Arecibo & Arecibo & Arecibo & Arecibo & Arecibo & Arecibo & GBT & GBT & GBT & GBT & Arecibo & Arecibo \\
\hline
J0023+0923    & \phn 0   & \phn 0   & \phn 4   &     18   & \phn 4   &     24   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   \\
J0030+0451    & \phn 0   & \phn 0   &     36   &     16   &     36   &     24   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   \\
J0340+4130    & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     26   & \phn 0   &     25   & \phn 0   & \phn 0   \\
J0613$-$0200  & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     40   &     47   &     42   &     45   & \phn 0   & \phn 0   \\
J0645+5158    & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     31   & \phn 0   &     29   & \phn 0   & \phn 0   \\
J0931$-$1902  & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     11   & \phn 0   & \phn 8   & \phn 0   & \phn 0   \\
J1012+5307    & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     45   &     49   &     45   &     47   & \phn 0   & \phn 0   \\
J1024$-$0719  & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 3   &     49   & \phn 8   &     47   & \phn 0   & \phn 0   \\
J1455$-$3330  & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     30   &     47   &     35   &     47   & \phn 0   & \phn 0   \\
J1600$-$3053  & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     25   &     48   &     26   &     43   & \phn 0   & \phn 0   \\
J1614$-$2230  & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 6   &     48   & \phn 8   &     43   & \phn 0   & \phn 0   \\
J1640+2224    & \phn 0   & \phn 0   &     42   &     18   &     42   &     23   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   \\
J1643$-$1224  & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     41   &     49   &     43   &     46   & \phn 0   & \phn 0   \\
J1713+0747    & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     46   &     24   &     40   &     52   &     41   &     48   &     42   &     24   \\
J1738+0333    & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 9   &     18   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 9   &     16   \\
J1741+1351    & \phn 0   & \phn 0   & \phn 6   &     14   &     20   &     20   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   \\
J1744$-$1134  & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     40   &     47   &     41   &     44   & \phn 0   & \phn 0   \\
J1747$-$4036  & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     24   & \phn 0   &     21   & \phn 0   & \phn 0   \\
J1832$-$0836  & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     10   & \phn 0   &     10   & \phn 0   & \phn 0   \\
J1853+1303    & \phn 0   & \phn 0   & \phn 5   &     13   &     30   &     20   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   \\
B1855+09      & \phn 0   & \phn 0   &     46   &     16   &     46   &     26   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   \\
J1903+0327    & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     16   &     18   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     16   &     17   \\
J1909$-$3744  & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     38   &     50   &     37   &     48   & \phn 0   & \phn 0   \\
J1910+1256    & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     50   &     23   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     21   &     16   \\
J1918$-$0642  & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     38   &     48   &     37   &     46   & \phn 0   & \phn 0   \\
J1923+2515    & \phn 0   & \phn 0   & \phn 5   &     12   & \phn 5   &     19   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   \\
B1937+21      & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     41   &     19   &     43   &     48   &     42   &     47   &     29   &     17   \\
J1944+0907    & \phn 0   & \phn 0   & \phn 8   &     14   &     24   &     20   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   \\
J1949+3106    & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     16   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     14   \\
B1953+29      & \phn 0   & \phn 0   & \phn 7   &     12   &     34   &     16   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   \\
J2010$-$1323  & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 6   &     48   & \phn 5   &     47   & \phn 0   & \phn 0   \\
J2017+0603    & \phn 0   & \phn 0   & \phn 0   & \phn 6   & \phn 0   &     24   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 1   &     18   \\
J2043+1711    & \phn 0   & \phn 0   & \phn 4   &     13   & \phn 4   &     18   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   \\
J2145$-$0750  & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     24   &     47   &     24   &     46   & \phn 0   & \phn 0   \\
J2214+3000    & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 2   &     22   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 4   &     19   \\
J2302+4442    & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   &     25   & \phn 0   &     24   & \phn 0   & \phn 0   \\
J2317+1439    &     45   &     22   &     45   &     18   & \phn 0   &     16   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   & \phn 0   \\
\hline
\end{tabular}
\end{table*}

